Non-uniform Blur Kernel Estimation via Adaptive Basis Decomposition

Motion blur estimation remains an important task for scene analysis and image restoration. In recent years, the removal of motion blur in photographs has seen impressive progress in the hands of deep learning-based methods, trained to map directly from blurry to sharp images. Characterization of the motion blur, on the other hand, has received less attention, and progress in model-based methods for deblurring lags behind that of data-driven end-to-end approaches. In this work we revisit the problem of characterizing dense, non-uniform motion blur in a single image and propose a general non-parametric model for this task. Given a blurry image, a neural network is trained to estimate a set of image-adaptive basis motion kernels as well as the mixing coefficients at the pixel level, producing a per-pixel motion blur field. We show that our approach overcomes the limitations of existing non-uniform motion blur estimation methods and leads to extremely accurate motion blur kernels. When applied to real motion-blurred images, a variational non-uniform blur removal method fed with the estimated blur kernels produces high-quality restored images. Qualitative and quantitative evaluation shows that these results are competitive or superior to results obtained with existing end-to-end deep learning (DL) based methods, thus bridging the gap between model-based and data-driven approaches.

==> latex/SANDBOX_oldText.tex <==

\section{Introduction - Old}


Motion blur results from the relative motion between the camera and the scene, which is determined by the interaction of three elements: the motion of the camera or egomotion, the three-dimensional geometry of the scene, and the motion of objects in the scene.  When the exposure time is large compared to the relative motion, the camera sensor at each point receives and accumulates light coming from different sources, producing different amounts of blur. 

Psychophysical and neurological evidence show that motion blur provides important cues for visual perception, scene understanding and locomotion~\cite{burton2015effect,harrington1981perception,royden2012use}. Besides deblurring, motion blur estimation has been successfully applied to different tasks such as scene interpretation, structure from motion, image segmentation, and uncertainty characterization of the observation ~\cite{favaro2004variational,strasdat2010efficient,ma1990depth}. \textcolor{olive}{Este paragrapho esta escrito con la idea de descentrarnos de deblurring. Queremos eso? o queremos centrarnos en que somos un metodo de non-blind deblurring?}

\textcolor{olive}{Deberiamos de dar 1 poco de bola a que casi todos los metodos de calculo de kernels son para casos uniformes? y asi motivar el calculo de metodos no uniformes, enfatizar los costos que son computacionalmente, por tanto se han utilizado metodos donde hacen una aproximacion mediante OF estimation o homography estimation, y luego venimos nosotros con nuestra super solucion! donde gracias a nuestra base de kernel adaptativa, somos capaces de calcular a dense kernel estimation, and overcoming the computational cost by using a low rank decomposition. }
Existing non-uniform motion blur estimation methods assume a parametric model of the motion field, either by considering a global parametric form induced by camera motion~\cite{gupta2010singleimage,hirsch2011fastremoval,dai2008motion, whyte2010nonuniform}, or  by locally modeling the motion field with linear kernels, parameterized by the length of the kernel support and its orientation
~\cite{gong2017motion,kim2014segmentation-free,dai2008motion,sun2015learning}. In most situations, for instance under camera shake from hand tremor, those models are do not generalize to real case scenarios~\cite{gavant2011physiological}.  \textcolor{olive}{Mas, general, en casos donde el movimiento no viene inducido solo por la camara, estos metodos no generalizan.}

We propose a novel approach for non-parametric, dense, spatially-varying motion blur estimation based on an efficient low-rank representation of the pixel-wise motion blur kernels \textcolor{olive}{able to deal with complex image deblurring problems}. More precisely, for each blurred image, a neural network estimates an image-specific set of kernel basis functions, as well as a set of pixel-wise mixing coefficients, cf. Figure~\ref{fig:pipeline}. In this way, for each pixel a unique motion blur kernel is assigned, given by the corresponding linear combination of the image-specific kernel basis functions. \textcolor{red}{We show that this procedure allows to generate a wide range of complex motion blur kernels that are well adapted to real acquisition scenarios.} \textcolor{olive}{Creo que no ensenamos the wide range of complex motion blur, lo que si que ensenamos es que los kernels se adaptan a todo tipo de imagenes, es decir que genralizan.} To the best of our knowledge, the proposed approach is the first dense non-parametric non-uniform motion blur estimation method.


To further validate our method, we apply our estimated motion blur fields  to two tasks: model-based image deblurring \cite{cho2009fast,kupyn2018deblurgan,kupyn2019deblurgan,xu2010two,whyte2010nonuniform} and blur detection \cite{golestaneh2017spatially,ma2018deep,shi2014discriminative}. We show that in both cases we achieve results that are comparable to those of state-of-the-art end-to-end deep learning methods in standard benchmarks of real blurred images, therefore contributing to bridge the gap between model-based and data-driven approaches.

Code and pre-trained model weights will be available upon acceptance.



